Beyond Training: Optimizing Reinforcement Learning Based Job Shop Scheduling Through Adaptive Action Sampling

Learned construction heuristics for scheduling problems have become increasingly competitive with established solvers and heuristics in recent years. In particular, significant improvements have been observed in solution approaches using deep reinforcement learning (DRL). While much attention has been paid to the design of network architectures and training algorithms to achieve state-of-the-art results, little research has investigated the optimal use of trained DRL agents during inference. Our work is based on the hypothesis that, similar to search algorithms, the utilization of trained DRL agents should be dependent on the acceptable computational budget. We propose a simple yet effective parameterization, called $\delta$-sampling that manipulates the trained action vector to bias agent behavior towards exploration or exploitation during solution construction. By following this approach, we can achieve a more comprehensive coverage of the search space while still generating an acceptable number of solutions. In addition, we propose an algorithm for obtaining the optimal parameterization for such a given number of solutions and any given trained agent. Experiments extending existing training protocols for job shop scheduling problems with our inference method validate our hypothesis and result in the expected improvements of the generated solutions.

==> tables/delta_values_table1.tex <==

\begin{table}
\centering
\begin{tblr}{
  cell{1}{3} = {c=3}{},
  cell{3}{1} = {r=4}{},
  cell{7}{1} = {r=4}{},
  hline{3,7} = {-}{},
  rowsep=0.5pt,
}
    &        & \hspace {20pt} sample size &       &     \\
    &        & 32          & 128   & 512               \\
L2G & 6x6    & 0.30        & 0.10  & 0.11              \\
    & 15x15  & 0.70        & 0.86  & 0.43              \\
    & 20x20  & 1.25        & 1.46  & 0.80              \\
    & 100x20 & 0.58        & 0.43  & \textasciitilde{} \\
L2D & 6x6    & 2.06        & 1.37  & 0.93              \\
    & 15x15  & 12.25       & 6.02  & 3.32              \\
    & 20x20  & 10.35       & 10.38 & 10.05             \\
    & 100x20 & 15x15       & 10.88 & \textasciitilde{} 
\end{tblr}
\end{table}
